Celeritas: GPU-accelerated particle transport for detector simulation in High Energy Physics experiments

Within the next decade, experimental High Energy Physics (HEP) will enter a new era of scientific discovery through a set of targeted programs recommended by the Particle Physics Project Prioritization Panel (P5), including the upcoming High Luminosity Large Hadron Collider (LHC) HL-LHC upgrade and the Deep Underground Neutrino Experiment (DUNE). These efforts in the Energy and Intensity Frontiers will require an unprecedented amount of computational capacity on many fronts including Monte Carlo (MC) detector simulation. In order to alleviate this impending computational bottleneck, the Celeritas MC particle transport code is designed to leverage the new generation of heterogeneous computer architectures, including the exascale computing power of U.S. Department of Energy (DOE) Leadership Computing Facilities (LCFs), to model targeted HEP detector problems at the full fidelity of Geant4. This paper presents the planned roadmap for Celeritas, including its proposed code architecture, physics capabilities, and strategies for integrating it with existing and future experimental HEP computing workflows.

==> sections/performance.tex <==
%%---------------------------------------------------------------------------%%
% performance.tex
%%---------------------------------------------------------------------------%%
\section{\celeritas performance}

Given the range of detector geometry complexities, primary event types, and
amount of output, there is no general case that provides a simple performance
number such as a simulation rate in events per second. Therefore, our ultimate
performance metric will be based on a set of real-world \acs{hep} detector
workflow use cases. \celeritas must run the targeted models at the same fidelity
as the current state-of-the-art but in much less time. In the next sections,  we
will present the two \acp{fom} that will be used to measure success, along with
a few preliminary performance results comparing \celeritas with current
state-of-the-art \ac{mc} codes.

% - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - %
\subsection{Performance metrics}

On \ac{lcf} hardware for the next decade, \acp{gpu} will provide the bulk of the
compute capability, so one critical performance metric is the ratio of the
runtime of \celeritas using \acp{gpu} to using only the \acp{cpu} of a given
machine. This \ac{fom} represents the ability of \celeritas to effectively use
the hardware that is available and must be sufficiently high to justify running
on \ac{lcf} resources. We will target a factor of $160\times$ for a single
\ac{gpu} to a single \ac{cpu}, which is the relative \ac{gpu}/\ac{cpu}
performance of the Shift \ac{mc} transport code
\cite{hamilton_continuous-energy_2019}.

A second performance metric is critical to the programmatic viability of
\celeritas in the broader \ac{hep} community: the work done for the same amount
of cost in power consumption and hardware, using Geant4 on \ac{cpu} as a
baseline. This \ac{fom} is the motivation for \ac{hep} workflows to adapt to
using \celeritas for \ac{mc} transport. The Geant4 team supposes that a factor
of two speedup resulting from ``adiabatic improvements'' to their code is not
outside the realm of possibility \cite{marc_verderi_geant4_2021}, so a $2
\times$ cost improvement of \celeritas runtime over Geant4 runtime is our second
target. Assuming that electricity consumption (and waste heat disposal) are the
primary constraints for independent \ac{hep} computing centers, this factor
should be evaluated by comparing the performance of Geant4 on \acp{cpu} with a
comparable power requirement as \celeritas on \acp{gpu}. At the present time,
for example, that comparison might be for an AMD 3rd Gen EPYC Processor power
(\SI{280}{\watt} for 64 cores) to a PCIe \nvidia A100 (\SI{250}{\watt} for 108
symmetric multiprocessors).

Meeting these \acp{fom} with Geant4-equivalent physics capabilities and
providing a solid user interface and \ac{io} integration to \ac{hep} workflows
will be the ultimate confirmation that \celeritas is a viable option for
\ac{hep} experiments. At this point \celeritas will be ideal for execution on
\ac{doe} \acp{lcf} and will be sufficiently fast on its own merits to motivate
independent adoption on capacity systems.

% - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - %
\subsection{Preliminary results}

The \celeritas team is developing a series of internal test problems to validate
every aspect of the code, including physics, geometry, \ac{em} fields, and
\ac{io}. Additionally, we are participating with the \acs{adept} project on a
series of common physics and performance benchmarks. Here, we present a small
set of preliminary results comparing \celeritas against Geant4 and \acs{adept}
using the \emph{TestEm3} benchmark test problem, available in \acs{adept}'s
repository\footnote {
    \url{https://github.com/apt-sim/AdePT}
}. This problem's geometry is composed of 50 rectangular layers, each
containing a Pb absorber and a liquid Ar gap.

In order to run a comparison between the three codes, we ported the
\acs{adept}'s implementation of the \emph{TestEm3} geometry to a Geant4
application, which in turn exported the geometry as a \acs{gdml} file that is
the current default input used by \celeritas. All three applications are running
the same physics models with the same secondary production thresholds.
Nevertheless, there are a few main caveats:
\begin{itemize}[itemsep=0pt]
    \item \celeritas and \acs{adept} use different \acp{prng};
    \item Geant4 uses its own navigation system, whereas \celeritas and
    \acs{adept} rely on \acs{vecgeom};
    \item \acs{adept} runs one event at a time, while celeritas loads and runs
    all primaries concurrently;
\end{itemize}

The results are produced using a particle-gun type input with \num{100000}, 10
GeV, electron primaries placed before the first layer. Their momentum direction
is fixed and pointed perpendicularly towards the layers. The compute node uses
the same \acp{gpu} as \ac{olcf}'s Summit: it has Intel Xeon Gold 5218 (Cascade
Lake) \acp{cpu} running at 2.3GHz (2 sockets of 16 cores with 2 hardware threads
per core, with \SI{188}{\giga\byte} total memory), and \nvidia V100 \acp{gpu}
(each with 80 symmetric multiprocessors, 64 CUDA cores per multiprocessor, and
\SI{16}{\giga\byte} memory). The current physics equivalency relies only on the
mean deposited energy per layer (Fig.~\ref{fig:testem3-edep}), which shows good
agreement between \acs{adept} and Geant4, with \celeritas being within a few
percent. Although the reason for this discrepancy still has to be fully
understood, it is likely caused by \celeritas' current linear interpolation of
energy-loss cross-section data. Geant's documentation explicitly states that for
accurate physics results, higher-order interpolations methods, such as
splined-based or log-log, are needed. The performance is measured in events per
second---where an event here is one primary particle---and presented in
Table~\ref{tab:testem3-performance}. \celeritas shows a speedup factor of
178$\times$ when compared to Geant4, and is approximately 3.3$\times$ faster
than \acs{adept}. For a serial \ac{cpu} run, \celeritas is about 1.6$\times$
faster than Geant4.

\begin{figure}
    \centering
    \includegraphics[width=0.7\textwidth]{figs/testem3_edep.pdf}
    \caption{Mean energy deposition per layer, represented by integer numbers
    in the $x$ axis. Each layer is composed by a pair of absorber and gap made
    of Pb and liquid Ar.}
    \label{fig:testem3-edep}
\end{figure}

\begin{table}
    \caption{Comparison between \celeritas, \acs{adept}, and Geant4 performances
    in events per second. The speedup factor is calculated with respect to
    Geant4.}
    \label{tab:testem3-performance}
    \centering
    \begin{tabular}{llrr}
        \toprule
        Application & Execution & Performance [events/s] & Speedup factor\\
        \midrule
        Geant4      & \ac{cpu} (serial) & 11.4   & 1.0\\
        \acs{adept} & \ac{gpu}          & 618.5  & 54.0\\
        \celeritas  & \ac{gpu}          & 2040.9 & 178.2\\
        \celeritas  & \ac{cpu} (serial) & 18.5   & 1.6\\
        \bottomrule
    \end{tabular}
  \end{table}

